Policy Learning with Abstention

Policy learning algorithms are widely used in areas such as personalized medicine and advertising to develop individualized treatment regimes. However, most methods force a decision even when predictions are uncertain, which is risky in high-stakes settings. We study policy learning with abstention, where a policy may defer to a safe default or an expert. When a policy abstains, it receives a small additive reward on top of the value of a random guess. We propose a two-stage learner that first identifies a set of near-optimal policies and then constructs an abstention rule from their disagreements. We establish fast O(1/n)-type regret guarantees when propensities are known, and extend these guarantees to the unknown-propensity case via a doubly robust (DR) objective. We further show that abstention is a versatile tool with direct applications to other core problems in policy learning: it yields improved guarantees under margin conditions without the common realizability assumption, connects to distributionally robust policy learning by hedging against small data shifts, and supports safe policy improvement by ensuring improvement over a baseline policy with high probability.

==> preamble.tex <==
\usepackage{amsmath,amsthm,mathtools,amssymb}

\usepackage{thmtools,thm-restate}
\usepackage{bbm}
\RequirePackage{algorithm}
\RequirePackage{algorithmic}
\usepackage{graphicx}
\usepackage{subcaption}

\usepackage{color,soul}
\usepackage{changepage}   % for adjustwidth
\usepackage[font=small,labelfont=bf]{caption}
% \captionsetup{aboveskip=2pt, belowskip=0pt}
% \usepackage{algorithm}
% \usepackage{algorithmic}
\usepackage[usenames,svgnames,xcdraw,table]{xcolor}
% \usepackage[left=2.0cm, right=2.0cm, top=2.3cm]{geometry}

\definecolor{amethyst}{rgb}{0.6, 0.4, 0.8}


\usepackage{url}
\usepackage[nameinlink,noabbrev,capitalise]{cleveref}
% \definecolor{DarkBlue}{rgb}{0.1,0.1,0.5}
% \definecolor{DarkGreen}{rgb}{0.1,0.5,0.1}
% \usepackage{hyperref}
% \hypersetup{
%    colorlinks   = true,
%  linkcolor    = DarkBlue, % color of internal links
%  urlcolor     = DarkBlue, % color of external links
% 	 citecolor    = DarkGreen % color of links to bibliography
% }
% \usepackage[capitalize]{cleveref}
% \usepackage{graphicx}
% \usepackage{svg}
% \usepackage{float}
% % \usepackage{verbatim}
% \usepackage{caption}

% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}{Lemma}
% \newtheorem{claim}[lemma]{Claim}
% \newtheorem{corollary}[lemma]{Corollary}
% \newtheorem{definition}{Definition}
% \newtheorem{observation}{Observation}
% \newtheorem*{example}{Example}
% \newtheorem{remark}{Remark}
% \newtheorem{proposition}[lemma]{Proposition}


% Convenience macros: filenames + trims (left bottom right top)
\newcommand{\baselinePlot}{figures/combined_baseline_optimality_gap_all_algorithms.png}
\newcommand{\noisePlot}{figures/combined_noise_variance_all_algorithms.png}
% Start with these; increase/decrease a few pt to taste after compiling
\newcommand{\trimA}{trim=16pt 12pt 14pt 18pt,clip} % baseline-gap figure
\newcommand{\trimB}{trim=16pt 12pt 14pt 18pt,clip} % noise-variance figure


\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\def\[#1\]{\begin{align*}#1\end{align*}}
% \def\[\*#1\*\]{\begin{align*}#1\end{align*}}
%%%%%%%%%%%%%%%%%%%%%%%THEOREMS

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
% \newtheorem*{lemma*}[theorem]{Lemma}
\newtheorem*{lemma*}{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{claim}[theorem]{Claim}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%MACROS
\newcommand{\f}[1]{\boldsymbol{#1}}
\newcommand{\bb}[1]{\mathbb{#1}}
\newcommand{\fl}[1]{\mathbf{#1}}
\newcommand{\ca}[1]{\mathcal{#1}}
\newcommand{\m}[1]{\mathrm{#1}}
\newcommand{\s}[1]{\mathsf{#1}}
\newcommand{\Reg}{\mathrm{Reg}}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\Su}{\mathsf{occ}}
\newcommand{\pj}[1]{\todo{PJ: #1}}
\newcommand{\lr}[1]{{\left|\left|#1\right|\right|}}
\newcommand{\bproof}{\bigskip {\bf Proof. }}
\newcommand{\eproof}{\hfill\qedsymbol}
\newcommand{\fac}{\Phi}
\newcommand{\welf}{\textsc{Wel-Alg}}
\newcommand{\alg}{\textsc{Alg}}
\newcommand{\Ttil}{\widetilde{\s{T}}}
\newcommand{\Td}{\s{T}'}
\newcommand{\T}{\s{T}}
\newcommand{\x}{\mathbf x}
\newcommand{\bX}{\mathbf X}
\newcommand{\bV}{\mathbf V}
\newcommand{\bA}{{\mathbf A}}
\newcommand{\bI}{{\mathbf I}}
\newcommand{\bH}{{\mathbf H}}
\newcommand{\bG}{{\mathbf G}}
\newcommand{\bW}{{\mathbf W}}
\newcommand{\bM}{{\mathbf M}}
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\cX}{{ \mathcal{X}}}

\newcommand{\ctX}{\widetilde{{ \mathcal{X}}}}
\newcommand{\cE}{{ \mathcal{E}}}
\newcommand{\cA}{{ \mathcal{A}}}
\newcommand{\cB}{{ \mathcal{B}}}
\newcommand{\cL}{{\mathcal{L}}}
\newcommand{\cD}{{\mathcal{D}}}
\newcommand{\cT}{{\mathcal{T}}}
\newcommand{\cR}{{\mathcal{R}}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\enet}{{ \mathcal{C}}_\varepsilon}
\newcommand{\opt}{\bm{\omega}}
\newcommand{\W}{\mathcal{W}}
\newcommand{\arm}{\mathtt{arm}}
\newcommand{\thta}{\theta^*}
\newcommand{\thth}{\widehat{\theta}}
\newcommand{\thtill}{\widetilde{\theta}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\R}{\mathbb{R}}

\newcommand{\prob}{\mathbb{P}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\NRg}{\textsc{NR}}
\newcommand{\Rg}{\textsc{R}}
\newcommand{\ex}{\mathrm{exp}}
\newcommand{\LNCB}{\mathrm{LNCB}}
\newcommand{\UNCB}{\mathrm{UNCB}}
\newcommand{\UCB}{\mathrm{UCB}}
\newcommand{\Sample}{S}
\newcommand{\norm}[2]{\left\lVert #1 \right\rVert_{#2}}
\newcommand{\sfT}{\s{T}}
\newcommand{\cvx}{\mathrm{cvh}}
\renewcommand{\l}{\left}
\renewcommand{\r}{\right}
\newcommand{\lrc}[1]{\left\{ #1 \right\}}
\newcommand{\lrb}[1]{\left[ #1 \right]}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}

\setlength{\parindent}{0pt}
\newcommand{\dotprod}[2]{\langle #1 ,#2 \rangle}
\newcommand{\nn}{\nonumber}
\newcommand{\pist}{{\pi^*}}
\newcommand{\pihat}{{\widehat{\pi}}}
\newcommand{\pitil}{{\widetilde{\pi}}}
\newcommand{\Pihat}{{\widehat{\Pi}}}
\newcommand{\Pitil}{{\widetilde{\Pi}}}
\newcommand{\tauh}{{\widehat{\tau}}}
\newcommand{\Vnq}{{V^q_n}}
\newcommand{\Vq}{{V^q}}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\xtil}{\widetilde{x}}
\newcommand{\ytil}{\widetilde{y}}
\newcommand{\mudp}[2]{\mud \left( \dotprod{#1}{#2} \right) }
\newcommand{\mup}[2]{\mu \left( \dotprod{#1}{#2} \right) }
\newcommand{\kap}{\kappa}
\newcommand{\kapst}{{\kappa^*}}
\newcommand{\kapav}{{\widehat{\kappa}}}
\newcommand{\const}{\textbf{c} \,}
%\newcommand{\detCond}{(1 + \textbf{ f })}
\newcommand{\detCond}{2}
\newcommand{\indic}[1]{\mathbbm{1}\!\!\l\{#1\r\}}
\newcommand{\sign}{\text{sign}}




% \makeatletter
% \newcommand*\defhatgreek[1]
%   {%
%     \expandafter\newcommand\expandafter*\csname h#1\endcsname
%       {\hat{\csname #1\endcsname}}%
%   }
% \@for\zz:=%
%   {%
%     alpha,beta,gamma,delta,epsilon,varepsilon,zeta,eta,theta,vartheta,kappa,%
%     lambda,mu,nu,xi,pi,varpi,rho,varrho,sigma,varsigma,tau,upsilon,phi,varphi,%
%     chi,psi,omega,%
%     Gamma,Delta,Theta,Lambda,Xi,Pi,Sigma,Upsilon,Phi,Psi,Omega%
%   }\do
%   {%
%     \expandafter\defhatgreek\expandafter{\zz}%
%   }



\newcommand{\dr}{\mathrm{DR}}
\newcommand{\err}{\mathrm{Err}}
\newcommand{\vdr}{V_\dr}
\newcommand{\vdrn}{V_{\dr,n}}
\newcommand{\vdrp}{V_\dr^{(p)}}
\newcommand{\vdrnp}{V_{\dr,n}^{(p)}}
\newcommand{\vp}{V^{(p)}}
\newcommand{\errdr}{\err_{\dr}}
\newcommand{\pifinal}{\pi_{\text{final}}}
\newcommand{\textred}[1]{{\textcolor{red}{#1}}}
\newcommand{\textblue}[1]{{\textcolor{blue}{#1}}}

\newcommand{\cXrem}{\cX_{rem}}

\def\DEBUG{true} % set this to be false to remove comments
	\ifdefined\DEBUG
\newcommand{\ayush}[1] {{\footnotesize\color{blue}[AS: #1]}}
